Distance Covariance in Metric Spaces: Non-Parametric Independence Testing in Metric Spaces (Master's thesis)

The aim of this thesis is to find a solution to the non-parametric independence problem in separable metric spaces. Suppose we are given finite collection of samples from an i.i.d. sequence of paired random elements, where each marginal has values in some separable metric space. The non-parametric independence problem raises the question on how one can use these samples to reasonably draw inference on whether the marginal random elements are independent or not. We will try to answer this question by utilizing the so-called distance covariance functional in metric spaces developed by Russell Lyons. We show that, if the marginal spaces are so-called metric spaces of strong negative type (e.g. seperable Hilbert spaces), then the distance covariance functional becomes a direct indicator of independence. That is, one can directly determine whether the marginals are independent or not based solely on the value of this functional. As the functional formally takes the simultaneous distribution as argument, its value is not known in the posed non-parametric independence problem. Hence, we construct estimators of the distance covariance functional, and show that they exhibit asymptotic properties which can be used to construct asymptotically consistent statistical tests of independence. Finally, as the rejection thresholds of these statistical tests are non-traceable we argue that they can be reasonably bootstrapped.

==> Characteristic_functions.tex <==



==> Distance_covariance.tex <==
\section{Distance Covariance - Original Article}
In this section we present the theory of the distance covariance statistics to measure dependence as introduced in \cite{Mikosch_dCorr_time_series}. The distance covariance introduced in \cite{szekely2007measuring} is a special case of the setup developed in \cite{Mikosch_dCorr_time_series}.

Primed random elements, denote an independent copy of the corresponding non-primed random element, and the Euclidean norm on $\bC$ and $\R^p$ for any $p\geq 1$ will all be denoted by $|\cdot|$ whenever the arguments space is clear, otherwise we will denote it by $|\cdot|$ and $|\cdot|_p$ respectively.
\subsection{Preliminaries}
Consider any measure space $(\cX,\cA,\mu)$ and $ 1 \leq p <\i$ and let
\begin{align*}
\cL^p_{\bC}\lp \mu \rp = \left\{ f:\cX \to \bC:  f\in \cM\left[ (\cX,\cA);(\bC,\cB(\bC))\right] ,\int_{\cX} |f|^p \, d\mu <\i  \right\},
\end{align*}
be the space of $p$-integrable, measurable, complex valued functions. The semi-norm $\| \cdot\|_p$ on $\cL^p_\bC(\mu)$ given by  $\|f\|_p = (\int_{\cX} |f|^p \, d\mu)^{1/p}$, can be used to construct the quotient vector-space $L^p_\bC(\mu)=\cL^p_\bC(\mu)/\mathrm{ker}(\|\cdot\|_p)$, that is the space of all equivalence classes of elements from $\cL^p_\bC(\mu)$ identified by the equivalence relation $f\sim g \iff f-g\in \mathrm{ker}(\|\cdot\|_p) \iff f=g \, \, \mu\text{-a.e}.$

The space of interest is especially $L^2_\bC(\mu)$ because this vector-space becomes a complete complex inner product space when equipped with the inner product $\la \cdot,\cdot \ra_{2}:L^2_\bC(\mu)\times L^2_\bC(\mu)\to \bC$ and naturally induced norm $\|\cdot \|_2$ defined by
\begin{align*}
\la f,g \ra_{2} = \int_\cX f(x) \, \overline{g(x)}  d\mu(x),
\end{align*}
 and
\begin{align*}
\| f \|_2= \sqrt{\la f,f \ra_{2}} =  \lp \int_{\cX} |f|^2 d \mu \rp^{\frac{1}{2}} 
\end{align*}
where the overline denotes the complex conjugate.  \\ \\
Now assume that $\mu$ is a measure on $(\R^{p+q},\cB(\R^{p+q}))$
\begin{definition}[Principal value integral] \label{defi_principal_value_integral}
Let $d\geq 1$ and $f:\R^d \to \bC$ be a measurable function such that $1_{A^d_\ep}f \in \mathcal{L}^1_{\bC}(\lambda^d)$ for any $\ep>0$, where $A^d_\ep = \R^d \setminus [B(0,\ep)\cup B(0,1/\ep)^c]$ is a $d$-dimensional annulus. We define the principal value integral of $f$ over $\R^d$ as
	\begin{align*}
	\mathrm{p.v.} \int_{\R^d} f(x) \, d\lambda^d(x) =\lim_{\ep \downarrow 0} \int_{A_\ep^d} f(x) \, d\lambda^d(x).
	\end{align*}
\end{definition}
As the Lebesgue integral is indifferent to changes of the integrands on integration measure null-sets, we may as in the regular integration theory also define the principal value integral of a $\lambda^d$-almost everywhere defined function, by redefining the function such that it is well-defined on the whole of $\R^d$. In the subsequent part of the thesis, such a redefinition is not mentioned but always done when dealing with either principal value- or Lebesgue integrals of $\lambda^d$-almost everywhere defined functions.

One might also note that if either $f:\R^d \to[0,\i]$ or $f\in\cL^1_\bC(\lambda^d)$ then Lebesgue's monotone or dominated convergence theorem yields that the principle value integral of $f$ coincides with the regular Lebesgue integral of $f$ over $\R^d$, i.e.
\begin{align*}
\mathrm{p.v.} \int_{\R^d} f(x) \, d\lambda^d(x) = \int_{\R^d} f(x) \, d\lambda^d(x).
\end{align*}
It is not difficult to expend some of the regular integral properties to the principal value integral, for example we may move complex constants outside the principal value integral, and we also have the addition rule  
\begin{align*}
\mathrm{p.v.}\int_{\R^d}f+g \,d\lambda^d=\mathrm{p.v.}\int_{\R^d}f \,d\lambda^d +\mathrm{p.v.}\int_{\R^d}g \, d\lambda^d,
\end{align*}
if both addends lies within $[-\i,\i)$ or $(-\i,\i]$ (to avoid expressions like $\pm \i \mp \i$). \textcolor{red}{rewrite this section more smoothly and formal} 
\begin{lemma}[Lemma 1 of  \cite{reference_lemma1} \& \cite{szekely2007measuring}] \label{Lemma1_SRB}
	If $0<\alpha<2$, then for all $x\in\R^d$
	\begin{align*}
	\int_{\R^d} \frac{1-\cos(t^\t x)}{|t|^{d+\alpha}_d} \, d\lambda^d(t) = C(d,\alpha)|x|_d^\alpha
	\end{align*}
	where
	\begin{align*}
	C(d,\alpha)= \frac{2\pi^{d/2}\Gamma(1-\alpha/2)}{\alpha2^\alpha\Gamma((d+\alpha)/2)}
	\end{align*}
	with $c_d=C(d,1)$ and $\Gamma(x)=\int_0^\i y^{x-1}e^{-y}dy$ being the complete gamma function.
\end{lemma}
\begin{p}
	See proof of Lemma 1 in \cite{reference_lemma1}.
\end{p}
Note that is the articles \cite{reference_lemma1} and \cite{szekely2007measuring} the above integral is referred to as a principle value integral, but since the integrand is non-negative the above Lebesgue integral coincides with its corresponding principal value integral.
\begin{corollary}
	For any $x\in\R^p$ and $y\in\R^q$ it holds that
	\begin{align*}
	\mathrm{p.v.}\int_{\R^p} \mathrm{p.v.}\int_{\R^q} \frac{1-e^{i(t,s)^\t (x,y)}}{c_pc_q |t|_p^{p+1}|s|^{q+1}_q} \, d\lambda^q(s)d\lambda^p(t) &= |x|_p|y|_q
		\end{align*}	
\end{corollary}
\begin{p}
	First we note that
	\begin{align*}
	1-e^{i(t,s)^\t(x,y)} =& 1- \cos(t^\t x + s^t y) -i\sin (t^\t x + s^\t y) \\
	=& 1- \cos t^\t x \cos s^t y + \sin t^\t x \sin s^\t y -i (\sin t^\t x \cos s^\t y + \cos t^\t x \sin s^\t y) \\
	=&(1-\cos t^\t x)(1-\cos s^\t y) + \cos t^\t x + \cos s^\t y-2\cos t^\t x  \cos s^\t y \\ 
	&+ \sin t^\t x \sin s^\t y -i (\sin t^\t x \cos s^\t y + \cos t^\t x \sin s^\t y) \\
	\end{align*}
	
\end{p}
\begin{definition}[Weighted $L^2_{\bC}$ norm]
	content...
\end{definition}
\subsection{Distance covariance}
Consider any two random vectors $X\in\R^p$ and $Y\in\R^q$. The objective of distance covariance is to draw inference on whether $X$ and $Y$ are independent, that is to test the hypothesis
\begin{align*}
H_0: X\independent Y \quad \quad \text{against} \quad \quad H_1: X \not \independent Y
\end{align*}
We start by presenting the theory developed by G. J. Szekely, M. L. Rizzo, and N. K. Bakirov in \cite{szekely2007measuring} and (their) subsequent articles \cite{szekely2009brownian}, \cite{szekely2012uniqueness} and \cite{szekely2013thedistancecorrelationttestofindepdenceinhighdimension}. \textcolor{red}{Check if used and all articles are included.} \\ \\
\textbf{START ON ARTICLE: }\\ \\
Now by the Cauchy-Schwarz inequality we get that
\begin{align*}
|\phi_{X,Y}(t,s)-\phi_X(t)\phi_Y(s)|^2 &=  | E ( e^{it^\intercal X}-\phi_X(t) ) ( e^{i t^\t Y}-\phi_Y(s) ) |^2  \\
&= | \langle  e^{it^\intercal X}-\phi_X(t), \overline{e^{i t^\t Y}-\phi_Y(s)} \rangle_{2} |^2\\
&\leq \|  e^{it^\t X}-\phi_X(t) \|_{2}^2 \| \overline{e^{i t^\t Y}-\phi_Y(s)} \|_{2}^2 \\
&= \| e^{it^\t X}-\phi_X(t) \|_{2}^2 \|e^{i t^\t Y}-\phi_Y(s) \|_{2}^2,
 \end{align*}
for any $(t,s)\in\R^p \times \R^q$. Now by the orthogonality
\begin{align*}
\la e^{it^\t X}-\phi_X(t),\phi_X(t)\ra_{2} &= \int_\Omega  \lp  e^{it^\t X(\omega)}-\phi_X(t)\rp \overline{\phi_X(t)} dP(\omega) \\
&= \overline{\phi_X(t)}\lp \phi_X(t)-\phi_X(t)\rp \\
&=0,
\end{align*}
the Pythagorean theorem for inner product spaces yields that
\begin{align*}
\| e^{it^\t X}-\phi_X(t)\|_{2}^2&=\|e^{it^\t X}\|_{2}^2- \|\phi_X(t)\|_{2}^2 \\
&= \int_{\Omega} |e^{it^\t X}|^2 dP - \int_{\Omega} |\phi_X(t)|^2 dP2 \\
&= 1- |\phi_X(t)|^2,
\end{align*}
with a similar result for second factor. Hence we have shown that
\begin{align}
|\phi_{X,Y}(t,s)-\phi_X(t)\phi_Y(s)|^2 \leq \lp 1- |\phi_X(t)|^2\rp\lp 1-|\phi_Y(s)|^2\rp
\end{align}
for any $(t,s)\in\R^p \times \R^q$. By \cref{properties_char} \cref{char_properties_simple}
\begin{align*}
|\phi_X(t)|^2 &= \phi_X(t)\phi_{X'}(-t) =E\lp e^{it^\t X}\rp E\lp e^{-it^\t X}\rp \\
&= E\lp e^{it^\t(X-X')}\rp = \phi_{X-X'}(t) = \int_{\Omega} \cos\lp t^\t x\rp dP_{X-X'}(x),
\end{align*}
where we used that $X\independent X'$ and that the distribution of $X-X'$ is symmetric around $0$, such that $\Im\phi_{X-X'}=0$ by \cref{properties_char} \cref{char_prooerties_sym} and a similar equality holds likewise for $|\phi_Y(s)|^2$. Hence by applying Tonelli's theorem repeatedly and Lemma 1 of \cite{reference_lemma1} we get
\begin{align*}
\int_{\R^p\times \R^q }& \frac{|\phi_{X,Y}(t,s)-\phi_X(t)\phi_Y(s)|^2}{c_pc_q|t|^{1+p}_p|s|^{1+q}_q}d\lambda^p\times \lambda^q(t,s) \\
&\leq \int_{\R^q }\int_{\R^p} \frac{\lp 1- |\phi_X(t)|^2\rp\lp 1-|\phi_Y(s)|^2\rp}{c_pc_q|t|^{1+p}_p|s|^{1+q}_q}d\lambda^p(t)d \lambda^q(s) \\
&=\int_{\R^q }\frac{ 1-E \cos \lp t^\t(X-X')\rp}{c_q|s|^{1+q}_q}d\lambda^q(s) \int_{\R^p} \frac{ 1- E \cos \lp s^\t(Y-Y')\rp}{c_p|t|^{1+p}_p}d\lambda^p(t) \\
&=E\lp \int_{\R^q }\frac{ 1- \cos \lp t^\t(X-X')\rp}{c_q|s|^{1+q}_q}d\lambda^q(s)\rp E\lp \int_{\R^p} \frac{ 1-  \cos \lp s^\t(Y-Y')\rp}{c_p|t|^{1+p}_p}d\lambda^p(t) \rp\\
&= E|X-X'|_pE|Y-Y'|_q \\
&\leq 4E|X|_pE|Y|_q \\
&<\i,
\end{align*}
if $X$ and $Y$ both have finite first moment, i.e $E|X|_p<\i$ and $E|Y|_q<\i$. Thus the following definitions are well-defined.
\begin{definition}[Distance Covariance, Variance \& Correlation]
	For any two random elements $X\in\R^p$ and $Y\in\R^q$ with finite first moment, the distance covariance between $X$ and $Y$ is defined as the non-negative real number\begin{align*}
	\dcov(X,Y) = \sqrt {\cV^2(X,Y)},
	\end{align*}
	and the distance variance of $X$ is defined by
	\begin{align*}
	\dvar(X)=\dcov(X,X),
	\end{align*}
	and finally the distance correlation between $X$ and $Y$ is defined by
	\begin{align*}
	\dcor(X,Y)= \frac{\dcov(X,Y)}{\sqrt{\dvar(X) \dvar(Y)}},
	\end{align*}
	whenever the denominator is positive and zero otherwise, where
	\begin{align*}
	\cV^2(X,Y)=\int_{\R^p\times \R^q} \frac{|\phi_{X,Y}(t,s)-\phi_X(t)\phi_Y(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q} d\lambda^p\times \lambda^q(t,s).
	\end{align*}
\end{definition}
	\subsection{Estimators and their properties}
	We are now going to a present moment estimator for the distance covariance of $X$ and $Y$ given $n$ i.i.d. samples of $(X,Y)$. Then we prove properties like strong consistency for these estimator. \\ \\ Let $
(X_1,Y_1),...,(X_n,Y_n)$ be independent and identically disttributed with $(X_1,Y_1) \eqd (X,Y)$. A moment estimator for the distance covariance based on these $n$-samples is easily obtained by replacing the characteristic functions in $\cV^2(X,Y)$ by the empirical counterparts, given by
\begin{align*}
\phi^n_{X}(t)= \frac{1}{n}\sum_{i=1}^n e^{it^\t X_i},\quad \quad \phi^n_{Y}(s)= \frac{1}{n}\sum_{i=1}^n e^{is^\t Y_i}, \quad \quad \phi_{X,Y}^n(t,s)=\frac{1}{n}\sum_{i=1}^n e^{i(t,s)^\t (X_i,Y_i)},
\end{align*}
and we easily get that $E(\phi_X^n(t))=\phi_X(t)$ and that
\begin{align*}
\phi^n_{X}(t) = \underbrace{\frac{1}{n}\sum_{i=1}^n \cos\lp t^\t X_i\rp}_{\convas E\cos\lp t^\t X\rp} + i \underbrace{\frac{1}{n}\sum_{i=1}^n \sin\lp t^\t X_i\rp}_{\convas E\sin\lp t^\t X\rp} \convas \phi_X(t)
\end{align*}
as $n$ tends to infinity, by strong law of large numbers and coordinate-wise limit equivalence. Hence the emperical characteristic functions are unbiased and strongly consistent estimators of the characteristic functions for fixed arguments. 
\begin{theorem} \label{theorem_estimator_equivalence}
	The estimator $\dcov_n(X,Y)$ (based on a $n$-size i.i.d. sample)  of $\dcov(X,Y)$ given by replacing the characteristic functions by the emperical characteristic functions has the following less complex representation
	\begin{align*}
	\dcov_n(X,Y) &=  \lp\int_{\R^p\times \R^q} \frac{|\phi_{X,Y}^n(t,s)-\phi_X^n(t)\phi_Y^n(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q} d\lambda^p\times \lambda^q(t,s)\rp^{1/2} \\
	&= \frac{1}{n^2}\sum_{i=1}^n \sum_{j=1}^n |X_i-X_j|_p |Y_i-Y_j|_q \cdots \cdots
	\end{align*}
\end{theorem}
	\begin{p}[of theorem 2.4]
	By the non-negativity of the integrand we can apply Tonelli's theorem and restate the regular Lebesgue integrals as the principal value integrals from \cref{defi_principal_value_integral}
	\begin{align*}
	&\int_{\R^p\times \R^q} \frac{|\phi_{X,Y}^n(t,s)-\phi_X^n(t)\phi_Y^n(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q} d\lambda^p \times \lambda^q (t,s)\\
	=& \int_{\R^q }\int_{\R^p} \frac{|\phi_{X,Y}^n(t,s)-\phi_X^n(t)\phi_Y^n(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q}d\lambda^p(t)d \lambda^q(s) \\
	=& \mathrm{p.v.}\int_{\R^q } \mathrm{p.v.}\int_{\R^p} \frac{|\phi_{X,Y}^n(t,s)-\phi_X^n(t)\phi_Y^n(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q}d\lambda^p(t)d \lambda^q(s).
	\end{align*}
    The idea is now to expand the fraction into a sum and use that if the pricipal value integrals of each addend is in either $[-\i,\i)$ or $(-\i,\i]$ then the sum of integrals of each addends coincide with the above integral.     
    Thus we note that with $X_{i,j}=X_i-X_j$ and $Y_{i,j}= Y_i-Y_j$ for any $i,j \in \{1,...,n\}$
	\begin{align*}
	|\phi^n_{X,Y}(t,s)-\phi^n_X(t)\phi^n_Y(s)|^2 =& \phi^n_{X,Y}(t,s) \bar{\phi}^n_{X,Y}(t,s) + \phi^n_X(t)\bar{\phi}^n_X(t)\phi^n_Y(s)\bar{\phi}^n_Y(s) \\
	&-\phi^n_{X,Y}(t,s)\bar{\phi}^n_X(t)\bar{\phi}^n_Y(s)- \bar{\phi}^n_{X,Y}(t,s)\phi^n_X(t)\phi^n_Y(s) \\
%	=&\phi^n_{X,Y}(t,s) \bar{\phi}^n_{X,Y}(t,s) + \phi^n_X(t)\bar{\phi}^n_X(t)\phi^n_Y(s)\bar{\phi}^n_Y(s) \\
%	&-2 \Re \phi^n_{X,Y}(t,s)\bar{\phi}^n_X(t)\bar{\phi}^n_Y(s). \\
    =&  \frac{1}{n^2} \lp \sum_{i=1}^{n} e^{i(t,s)^t(X_i,Y_i)}\rp \lp \sum_{j=1}^{n} e^{-i(t,s)^t(X_j,Y_j)}\rp  \\
    &+ \frac{1}{n^4} \lp \sum_{i=1}^{n} e^{i t^t X_i}\rp \lp \sum_{j=1}^{n} e^{-i t^t X_j}\rp \lp \sum_{k=1}^{n} e^{i s^t Y_k}\rp \lp \sum_{l=1}^{n} e^{-i s^t Y_l}\rp \\
    &- \frac{1}{n^3} \lp \sum_{i=1}^n e^{i (t,s)^\t (X_i,Y_i)}\rp \lp \sum_{j=1}^{n} e^{-i t^t X_j}\rp \lp \sum_{k=1}^{n} e^{-i s^t Y_k}\rp \\
    &-\frac{1}{n^3} \lp \sum_{i=1}^n e^{-i (t,s)^\t (X_i,Y_i)}\rp \lp \sum_{j=1}^{n} e^{i t^t X_j}\rp \lp \sum_{k=1}^{n} e^{i s^t Y_k}\rp \\
	=&+ \frac{1}{n^2} \sum_{i,j=1}^n  e^{i(t,s)^\t (X_{i,j},Y_{i,j})} +   \frac{1}{n^4} \sum_{i,j,k,l=1}^n  e^{i(t,s)^\t (X_{i,j},Y_{k,l} ) }   \\
	&- \frac{1}{n^3} \sum_{i,j,k=1}^n  e^{i(t,s)^\t(X_{i,j},Y_{i,k})} - \frac{1}{n^3} \sum_{i,j,k=1}^n  e^{i(t,s)^\t(X_{i,k},Y_{j,k})}
	\end{align*}
	Add and subtract 1 to each term to get
	\begin{align*}
	|\phi^n_{X,Y}(t,s)-\phi^n_X(t)\phi^n_Y(s)|^2 =& -\frac{1}{n^2} \sum_{i,j=1}^n  1- e^{i(t,s)^\t (X_{i,j},Y_{i,j})} -   \frac{1}{n^4} \sum_{i,j,k,l=1}^n 1- e^{i(t,s)^\t (X_{i,j},Y_{k,l} ) }   \\
	& +\frac{1}{n^3} \sum_{i,j,k=1}^n 1- e^{i(t,s)^\t(X_{i,j},Y_{i,k})} + \frac{1}{n^3} \sum_{i,j,k=1}^n  1-e^{i(t,s)^\t(X_{i,k},Y_{j,k})} 
	\end{align*}
	Using that \textbf{(Prove this)}
		\begin{align*}
		\mathrm{p.v.}\int_{\R^p} \mathrm{p.v.}\int_{\R^q} \frac{1-e^{i(t,s)^\t (x,y)}}{c_pc_q |t|_p^{p+1}|s|^{q+1}_q} \, d\lambda^q(s)d\lambda^p(t) &=|x|_p|y|_q
		\end{align*}	

		we get that
		\begin{align*}
		&\int_{\R^p\times \R^q} \frac{|\phi_{X,Y}^n(t,s)-\phi_X^n(t)\phi_Y^n(s)|^2}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q} d\lambda^p \times \lambda^q (t,s)  \\ =& -\frac{1}{n^2} \sum_{i,j=1}^n |X_i-X_j|_p|Y_i-Y_j|_q -   \frac{1}{n^4} \sum_{i,j,k,l=1}^n |X_i-X_j|_p|Y_k-Y_l|_q   \\
		& +\frac{1}{n^3} \sum_{i,j,k=1}^n  |X_i-X_j|_p|Y_i-Y_k|_q + \frac{1}{n^3} \sum_{i,j,k=1}^n  |X_i-X_k|_p|Y_j-Y_k|_q \\
		=& -\frac{1}{n^2} \sum_{i,j=1}^n|X_i-X_j|_p|Y_i-Y_j|_q -   \frac{1}{n^4} \sum_{i,j,k,l=1}^n  |X_i-X_j|_p|Y_k-Y_l|_q   \\
		& +\frac{2}{n^3} \sum_{i,j,k=1}^n  |X_i-X_j|_p|Y_i-Y_k|_q 
		\end{align*}
\end{p}
	\newpage	
	Using Eulers formula  we get
	\begin{align*}
	&\phi^n_{X,Y}(t,s) \bar{\phi}^n_{X,Y}(t,s)\\
	=& \lp \frac{1}{n}\sum_{i=1}^n e^{i (t,s)^\t(X_i,Y_i)} \rp\lp \frac{1}{n}\sum_{j=1}^n e^{-i (t,s)^\t(X_j,Y_j)} \rp \\
	=& \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n e^{i (t,s)^\t(X_i,Y_i)-i (t,s)^\t(X_j,Y_j)}= \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n e^{i (t,s)^\t (X_{i,j},Y_{i,j})} \\
	=& \frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n \cos(t,s)^\t (X_{i,j},Y_{i,j}) + i \sin (t,s)^\t (X_{i,j},Y_{i,j}), \\
	=& 	\frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n \cos \lp t^\t X_{i,j}+s^\t Y_{i,j}\rp \\
	=& 	\frac{1}{n^2}\sum_{i=1}^n\sum_{j=1}^n \cos t^\t X_{i,j}  \cos s^\t Y_{i,j} - \sin t^\t X_{i,j}  \sin s^\t Y_{i,j} 
	\end{align*}
	where we in the third equality used that $\Im \lp \phi_{X,Y}^n(t,s)\bar{\phi}_{X,Y}^n(t,s)\rp=\Im|\phi_{X,Y}(t,s)|^2 =0$. Since 
	$t\mapsto \sin t^\t X_{i,j} / |t|^{p+1}_p$ is a odd function we get that
	\begin{align*}
	\int_{A^p_\ep}  \frac{\sin t^\t X_{i,j}  \sin s^\t Y_{i,j} }{c_pc_q |t|^{p+1}_p|s|^{q+1}_q}d\lambda^p(t) &= \frac{\sin s^\t Y_{i,j} }{c_pc_q |s|^{q+1}_q}\int_{A_\ep^p}  \frac{\sin t^\t X_{i,j}  }{ |t|^{p+1}_p}d\lambda^p(t) =0,
	\end{align*}
	hence
	\begin{align*}
	\mathrm{p.v.}\int_{\R^q } \mathrm{p.v.}\int_{\R^p} \frac{- \sin t^\t X_{i,j}  \sin s^\t Y_{i,j}}{c_pc_q |t|^{p+1}_p|s|^{q+1}_q}d\lambda^p(t)d \lambda^q(s)= 0
	\end{align*}
	\newpage
	\section{Distance Covariance - Mikosch Article Notes}
Now assume that $\mu$ is a measure on $(\R^{p+q},\cB(\R^{p+q}))$ such that it is finite on sets of the form
\begin{align*}
D_\delta = \{ (t,s)\in\R^p \times \R^q : |t|\land |s|>\delta \}, \quad \delta>0
\end{align*}

==> Notation.tex <==
\section{Notation}
$\mathcal{J}(\R^k)$ denotes the set of half-open rectangles in $\R^k$, that is
\begin{align*}
\mathcal{J}(\R^k) = \{ [a_1,b_1)\times \cdots \times [a_k,b_k) : a_i,b_i\in\R \, \forall i \}
\end{align*}

